On the Convergence of Reinforcement Learning in Nonlinear Continuous State Space Problems

We consider the problem of Reinforcement Learning for nonlinear stochastic dynamical systems. We show that in the RL setting, there is an inherent ``Curse of Variance" in addition to Bellman's infamous ``Curse of Dimensionality", in particular, we show that the variance in the solution grows factorial-exponentially in the order of the approximation. A fundamental consequence is that this precludes the search for anything other than ``local" feedback solutions in RL, in order to control the explosive variance growth, and thus, ensure accuracy. We further show that the deterministic optimal control has a perturbation structure, in that the higher order terms do not affect the calculation of lower order terms, which can be utilized in RL to get accurate local solutions.

==> A_Near_Optimal_Decoupling_Principle.tex <==
\section{A NEAR OPTIMAL DECOUPLING PRINCIPLE}\label{sec3}
%We discuss in detail the decoupling principle described in Section~\ref{section:decoupling}.
\textcolor{red}{Raman: We do not need this Section anymore.}
In this section, we outline a result that shows that the optimal deterministic feedback solution is near-optimal to the optimal solution to the stochastic problem to the fourth order in a small noise parameter $\epsilon$. Next, we show the perturbation structure of the optimal deterministic feedback law analogous to the PPE equation \eqref{PPE}. Putting these two results together, we show how we can obtain near optimal solutions to the optimal stochastic control problem, while ensuring accuracy and computational tractability, at least locally. We cover only the model based case, for the sake of brevity, and the RL based case is the subject of a comprehensive companion paper \cite{D2C2.0}.\\


We assume that the dynamics can be written in the control affine form 
$%$\begin{align} 
%\label{eq.0.1}
%\label{eq:dynamics1}
x_{t+1} = f(x_t) + g(x_t) u_t + \epsilon w_t, 
$%\end{align}
where $\epsilon < 1$ is a small parameter. We also assume that the instantaneous cost $c(\cdot, \cdot)$ has the following simple form, $c(x,u) = l(x) + \frac{1}{2} u'Ru.$
We emphasize that these assumptions,  quadratic control cost and affine in control dynamics, are typically satisfied.
In the following subsections, we first characterize the performance of any feedback policy. Then, we use this characterization to provide an $O(\epsilon^4)$ near-optimality result in the subsequent subsection.

%With a slight abuse of notation, let $\pi^{*} = \pi = (\pi_{t})^{T}_{t=1}$ be the optimal control law given by \eqref{cost_sto_orig} according to the dynamics \eqref{eq.0.1} and instantaneous cost \eqref{eq:cost1}.   

\subsection{Characterizing the Performance of a Feedback Policy}

Consider a noiseless  version of the system dynamics above. Denote the ``nominal'' state trajectory as $\bar{x}_{t}$ and the ``nominal'' control as $\bar{u}_{t}$ where $\bar{u}_{t} = \pi_{t}(\bar{x}_{t})$, and $\pi = (\pi_{t})^{T-1}_{t=1}$ is a given control policy. The resulting dynamics  without noise is given by $\bar{x}_{t+1} = f(\bar{x}_t) + g(\bar{x}_t) \bar{u}_t$.   

%Let the associated nominal incremental costs be denoted by $\bar{c}_t = l(\bar{x}_t) + \frac{1}{2} \bar{u}_t'R\bar{u}_t$, and the associated nominal terminal cost be denoted by $\bar{c}_T = c_T(\bar{x}_T)$. 

Assuming that $f(\cdot), g(\cdot)$ and $\pi_{t}(\cdot)$ are sufficiently smooth, we can expand the dynamics about the nominal trajectory. Denoting  $\delta x_t = x_t - \bar{x}_t, \delta u_t = u_t - \bar{u}_t$, we can express, 
\begin{align}
\delta x_{t+1} &= A_t \delta x_t + B_t \delta u_t + S_t(\delta x_t) + \epsilon w_t, %\label{eq2}\\
\delta u_{t} =  K_t \delta x_t + \tilde{S}_t(\delta x_t), \label{eq2}
\end{align}
where $A_t = \frac{\partial f}{\partial x}|_{\bar{x}_t} + \frac{\partial g\bar{u}_t}{\partial x}|_{\bar{x}_t}$, $B_t = g(\bar{x}_t)$, $K_{t} = \frac{\partial \pi_{t}}{\partial x}|_{\bar{x}_t}$, and  $S_t(\cdot), \tilde{S}_t(\cdot)$ are second and higher order terms in the respective expansions. Similarly, we can linearize the instantaneous cost $c(x_{t}, u_{t})$ about the nominal values $(\bar{x}_{t}, \bar{u}_{t})$ as,
\begin{align}
c(x_t,u_t) &= {l}(\bar{x}_{t}) + L_t \delta x_t + H_t(\delta x_t) + %\nonumber\\ 
\frac{1}{2}\bar{u}_t'R\bar{u}_t +  \delta u_t'R\bar{u}_t + \frac{1}{2}\delta u_t'R\delta u_t,\label{eq4}\\
c_{T}(x_{T}) &= {c}_{T}(\bar{x}_{T}) + C_T \delta x_T + H_T(\delta x_T),\label{eq5}
\end{align}
where $L_t = \frac{\partial l}{\partial x}|_{\bar{x}_t}$, $C_T  = \frac{\partial c_T}{\partial x}|_{\bar{x}_t}$, and $H_t(\cdot)$ and $H_T(\cdot)$ are second and higher order terms in the respective expansions.

Using \eqref{eq2}, we can write the closed loop dynamics  of the trajectory $(\delta x_{t})^{T}_{t=1}$ as, 
\begin{align}
\label{eq6}
\delta x_{t+1} = \underbrace{(A_t+B_tK_t)}_{\bar{A}_t} \delta x_t + \underbrace{\{B_t\tilde{S}_t(\delta x_t) + S_t(\delta x_t)\}}_{\bar{S}_t(\delta x_t)} + \epsilon w_t, 
\end{align} 
where $\bar{A}_t$ represents the linear part of the closed loop systems and the term $\bar{S}_t(\cdot)$ represents the second and higher order terms in the closed loop system. Similarly, the closed loop incremental cost given in  \eqref{eq4} can be expressed as
$%$\begin{align}
 %\label{eq7}
c(x_t,u_t) = \underbrace{\{{l}(\bar{x}_{t}) + \frac{1}{2}\bar{u}_t'R\bar{u}_t\}}_{\bar{c}_t} + \underbrace{[L_t + \bar{u}_t'RK_t]}_{\bar{C}_t} \delta x_t %\nonumber\\
+ \underbrace{\frac{1}{2}(K_t\delta x_t+\tilde{S}_t(\delta x_t))'R(K_t\delta x_t + \tilde{S}_t(\delta x_t)) + \bar{u}_t' R \tilde{S}_t(\delta x_t)}_{\bar{H}_t(\delta x_t)}. 
$%\end{align}

Therefore, the cumulative cost of any given closed loop trajectory $(x_{t}, u_{t})^{T}_{t=1}$  can be expressed as,
$%$\begin{align}
%\label{eq9a}
J^{\pi} = \sum^{T-1}_{t=1}c(x_{t}, u_{t} = \pi_{t}(x_{t})) + c_{T}(x_{T}) %\nonumber \\
=\sum_{t=1}^T \bar{c}_t + \sum_{t=1}^T \bar{C}_t \delta x_t + \sum_{t=1}^T \bar{H}_t(\delta x_t),
$%\end{align}
where $\bar{c}_{T} = c_{T}(\bar{x}_{T}),  \bar{C}_{T} = C_{T}$.

We first show the following critical result. 
\begin{lemma} 
\label{L1}
Given any sample path, the state perturbation equation 
%\[\delta x_{t+1} = \bar{A}_{t}  \delta x_{t} + \bar{S}_t(\delta x_t) + \epsilon w_t \]
given can be equivalently characterized  as
\begin{align}
\label{eq:mod-pert-1}
\delta x_{t}  = \delta x_t^l + e_t, ~ \delta x_{t+1}^l = \bar{A}_t \delta x_t^l + \epsilon w_t
\end{align} 
where $e_t$ is an $O(\epsilon^2)$ function that depends on the entire noise history $\{w_0,w_1,\cdots w_t\}$ and $\delta x_t^l$ evolves according to the  linear closed loop system. Furthermore, $e_t = e_t^{(2)} + O(\epsilon^3)$, where $e_t^{(2)} = \bar{A}_{t-1} e_{t-1}^{(2)} + \delta x_t^{l'}\bar{S}_{t-1}^{(2)} \delta x_t^l$, $e_0^{(2)} = 0$, and $\bar{S}_t^{(2)}$ represents the Hessian corresponding to the Taylor series expansion of the function $\bar{S}_t(\cdot)$. 
\end{lemma}



%Using  \eqref{eq:mod-pert-1} in  \eqref{eq.9a}, we can obtain the cumulative cost of any given closed loop trajectory as,
%\begin{align}
%J^{\pi} = \underbrace{\sum_{t=1}^T \bar{c}_t }_{\bar{J}^{\pi}} + \underbrace{\sum_{t=1}^T \bar{C}_t \delta x_t^l}_{\delta J_1^{\pi}} + %\nonumber\\
%\underbrace{\sum_{t=1}^T \bar{H}_t(\delta x_t) + \bar{C}_t \bar{\bar{S}}_t}_{\delta J_2^{\pi}}. \label{eq.9b}
%\end{align}
Next, we have the following result for the expansion of the cost to go function $J^{\pi}$.
\begin{lemma}
\label{L2}
Given any sample path, the cost-to-go under a policy can be expanded as: 
\begin{equation} 
J^{\pi}  = \underbrace{\sum_t \bar{c}_t}_{\bar{J}^{\pi}} + \underbrace{\sum_t \bar{C}_t \delta x_t^l}_{\delta J_1^{\pi}} + \underbrace{\sum_t \delta x_t^{l'}\bar{H}_t^{(2)} \delta x_t^l+ \bar{C}_t e_t^{(2)}}_{\delta J_2^{\pi}} + O(\epsilon^3),
\end{equation}
where $\bar{H}_t^{(2)}$ denotes the second order coefficient of the Taylor expansion of $\bar{H}_t(\cdot)$.
\end{lemma}


A consequence of the result above is the following. Suppose that given a policy $\pi_t(\cdot)$, we only consider the linear part, i.e., the linear approximation $\pi_t^l(x_t) = \bar{u}_t + K_t\delta x_t$. However, according to Lemma \ref{L2}, the $\epsilon^2$ terms in the expansion of the cost of any sample path solely result from the linear closed loop system. Therefore, it follows that the sample path cost under the full policy $\pi_t(\cdot)$ and the linear policy $\pi_t^l(\cdot)$ agree up to the $\epsilon^2$ term. Therefore, it follows that $E[J^{\pi}] - E[J^{\pi^l}]  = O(\epsilon^4)$. We summarize this result in the following:

%\begin{comment}
\begin{proposition}
\label{prop2}
Let $\pi_t(\cdot)$ be any given feedback policy. Let $\pi_t^l(x_t) = \bar{u}_t + K_t\delta x_t$ be the linear approximation of the policy. Then, the error in the expected cost to go under the two policies, $E[J^{\pi}] - E[J^{\pi^l}]  = O(\epsilon^4)$.
\end{proposition}

The above result forms the basis of the $O(\epsilon^4)$ decoupling result in the following subsection.
%\end{comment}

\subsection{An $O(\epsilon^4)$ Near-Optimal Decoupled Approach for Closed Loop Control} \label{Oe4}
In order to derive the results in this section, we need some additional structure on the dynamics. \textit{In essence, the results in this section require that the time discretization of the dynamics be small enough}. Thus, let the dynamics be given by:
\begin{equation}\label{SDE0}
x_t = x_{t-1} + \bar{f}(x_{t-1}) \Delta t + \bar{g}(x_{t-1}) u_t \Delta t + \epsilon \omega_t \sqrt{\Delta t},
\end{equation}
where $\omega_t$ is a white noise sequence, and the sampling time $\Delta t$ is small enough that $O(\Delta t^{\alpha})$ is negligible for $\alpha > 1$. The noise term above is a Brownian motion, and hence the $\sqrt{\Delta t}$ factor. Further, the incremental cost function $c(x,u)$ is given as:
$c(x,u) = \bar{l}(x) \Delta t + \frac{1}{2} u'\bar{R}u \Delta t.$
The main reason to use the above assumptions is to simplify the Dynamic Programming (DP) equation governing the optimal cost-to-go function of the system. The DP equation for the above system is given by:
\begin{equation}\label{DP}
J_t(x) = \min_{u_t} \{c(x,u) + E[J_{t+1}(x')]\},
\end{equation}
where $x' = x + \bar{f}(x)\Delta t + \bar{g}(x) u_t \Delta t + \epsilon \omega_t \sqrt{\Delta t}$ and $J_t(x)$ denotes the cost-to-go of the system given that it is at state $x$ at time $t$. The above equation is marched back in time with terminal condition $J_T(x) = c_T(x)$, and $c_T(\cdot)$ is the terminal cost function. Let $u_t(\cdot)$ denote the corresponding optimal policy. Then, it follows that the optimal control $u_t$ satisfies (since the argument to be minimized is quadratic in $u_t$)
\begin{equation}\label{opt_control}
u_t= -R^{-1}\bar{g}' J_{t+1}^x,
\end{equation}
where $J_{t+1}^x = \frac{\partial J_{t+1}}{\partial x}$.
 Further, let $u_t^d(\cdot)$ be the optimal control policy for the deterministic system, i.e., Eq. \ref{SDE0} with $\epsilon =0$. The optimal cost-to-go of the deterministic system, $\phi_t(\cdot)$ satisfies the deterministic DP equation:
\begin{equation}\label{detDP}
    \phi_t(x)= \min_{u}[c(x,u) + \phi_{t+1}(x')],
\end{equation}
where $x' = x + \bar{f}(x')\Delta t + \bar{g}(x')u\Delta t$. Then, identical to the stochastic case, $u_t^d = R^{-1}\bar{g}'\phi_t^x$.
Next, let $\varphi_t(\cdot)$ denote the cost-to-go of the deterministic policy when applied to the stochastic system, i.e., $u_t^d$ applied to Eq. \ref{SDE0} with $\epsilon > 0$. The cost-to-go $\varphi_t(\cdot)$ satisfies the policy evaluation equation:
\begin{equation}\label{detDP_eps}
   \varphi_t(x) = c(x, u_t^d(x)) + E[\varphi_{t+1}(x')],
\end{equation}
where now $x' = x+ \bar{f}(x)\Delta t + \bar{g}(x)u_t^d(x) \Delta t + \epsilon \omega_t \sqrt{\Delta t}$.
Note the difference between the equations \ref{detDP} and \ref{detDP_eps}.
Then, we have the following important result.
\begin{proposition}
\label{prop_eps}
The difference between the cost function of the optimal stochastic policy, $J_t$, and the cost function of the ``deterministic policy  applied to the stochastic system", $\varphi_t$, is $O(\epsilon^4)$, i.e. $|J_t (x) - \varphi_t (x)| = O(\epsilon^4)$ for all $(t,x)$.
\end{proposition}
The above result was originally proved in a seminal paper \cite{fleming1971stochastic} for first passage problems. We provide a simple derivation of the result for a final value problem below. \\


Given some initial condition $x_0$, consider a linear truncation of the optimal deterministic policy, i.e., let $u_t^l(\cdot) = \bar{u}_t + K_t\delta x_t$, where the deterministic policy is given by $u_t^d = \bar{u}_t + K_t\delta x_t + S_t(\delta x_t)$, where $S_t(\cdot)$ denote the second and higher order terms in the optimal deterministic feedback policy.  Using Proposition \ref{prop2}, it follows that the cost of the linear policy, say $\varphi_t^l(\cdot)$,  is within $O(\epsilon^4)$ of the cost of the deterministic policy $u_t^d(\cdot)$, when applied to the stochastic system in Eq. \ref{SDE0}. However, the result in Proposition \ref{prop_eps} shows that the cost of the deterministic policy is within $O(\epsilon^4)$ of the optimal stochastic policy. Taken together, this implies that the cost of the linear deterministic policy is within $O(\epsilon^4)$ of the optimal stochastic policy. This may be summarized in the following result.
\begin{proposition} \label{e4}
Let the optimal cost function under the true stochastic policy be given $J_t(\cdot)$ Let the optimal deterministic policy be given by $u_t^d(x_t) = \bar{u}_t + K_t\delta x_t + S_t(\delta x_t)$, and the linear approximation  to the policy be $u_t^l(x_t) = \bar{u}_t + K_t\delta x_t$, and let the cost of the linear policy be given by $\varphi_t^l(x)$. Then $|J_t(x) - \varphi_t^l(x)| = O(\epsilon^4)$ for all $(t,x)$.
\end{proposition}
Now, it remains to be seen how to design the $\bar{u}_t$ and the linear feedback term $K_t$. 
The open loop optimal control sequence $\bar{u}_t$ is found identically to the previous section. However, the linear feedback gain $K_t$ is calculated in a slightly different fashion and may be done as shown in the following.\\

We will use the classical Method of Characteristics to derive the result \cite{Courant-Hilbert}. Let us recall the Hamilton-Jacobi-Bellman (HJB) equation in continuous time under the same assumptions as above, i.e., quadratic in control cost $c(x,u) = l(x) + \frac{1}{2}r u^2$, and affine in control dynamics $\dot{x} = f(x) + g(x)u$, (the discrete time case for a sufficiently small discretization time then follows immediately, see Remark \ref{T-PFC-remarks}):
\begin{equation}
    \frac{\partial J}{\partial t} + l - \frac{1}{2}\frac{g^2}{r} J_x^2 + fJ_x = 0,
\end{equation}
where $J = J_t (x_t), \; J_x = \frac{\partial J}{\partial x_t}$, and the equation is integrated back in time with terminal condition $J_T(x_T) = c_T(x_T)$. Define $\frac{\partial J}{\partial t} = p, \; J_x= q$, then the HJB can be written as $F(t,x,J,p,q) =0$, where $F(t,x,J,p,q) = p+l -\frac{1}{2}\frac{g^2}{r}q^2 + fq$. One can now write the Lagrange-Charpit equations \cite{Courant-Hilbert} for the HJB as:
\begin{align}\label{L-C-1}
    \dot{x} = F_q = f -\frac{g^2}{r}q, \\
    \dot{q} = -F_x -qF_J = -l^x + \frac{gg^x}{r}q^2 - f^xq,\label{L-C-2}
\end{align}
with the terminal conditions $x(T) = x_T, \; q(T) = c_T^x(x_T)$, where $F_x = \frac{\partial F}{\partial x}$, $F_q = \frac{\partial F}{\partial q}$, $g^x = \frac{\partial g}{\partial x}$, $l^x = \frac{\partial l}{\partial x}$, $f^x = \frac{\partial f}{\partial x}$ and $c_T^x = \frac{\partial c_T}{\partial x}$.\\
Given a terminal condition $x_T$, the equations above can be integrated back in time to yield a characteristic curve of the HJB PDE. Now, we show how one can use these equations to get a local solution of the HJB, and consequently, the feedback gain $K_t$.\\ Suppose now that one is given an optimal nominal trajectory $\bar{x}_t$, $t \in [0,T]$ for a given initial condition $x_0$, from solving the open loop optimal control problem. Let the nominal terminal state be $\bar{x}_T$. We now expand the HJB solution around this nominal optimal solution. To this purpose, let $x_t = \bar{x}_t + \delta x_t$, for $t\in [0,T]$. Then, expanding the optimal cost function around the nominal yields: $J(x_t) = \bar{J}_t + G_t\delta x_t + \frac{1}{2}P_t\delta x_t^2+\cdots,$ where $\bar{J}_t = J_t(\bar{x}_t), G_t = \frac{\partial J}{\partial x_t}|_{\bar{x}_t}, P_t = \frac{\partial^2 J}{\partial x_t^2}|_{\bar{x}_t}$. Then, the co-state $q = \frac{\partial J}{\partial x_t} = G_t + P_t \delta x_t + \cdots$. For simplicity, we assume that $g^x = 0$ (this is relaxed but at the expense of a rather tedious derivation and we will `only state' the result for the general case at the end of this Section). Hence, 
\begin{align}
    \underbrace{\frac{d}{dt} (\bar{x}_t + \delta x_t)}_{\dot{\bar{x}}_t + \dot{\delta x}_t} = \underbrace{f(\bar{x}_t+ \delta x_t)}_{(\bar{f}_t + \bar{f}_t^x \delta x_t+\cdots)} - \frac{g^2}{r}(G_t + P_t \delta x_t+\cdots),
\end{align}
where $\bar{f}_t = f(\bar{x}_t), \bar{f}_t^x = \frac{\partial f}{\partial x_t}|_{\bar{x}_t}$. Expanding in powers of the perturbation variable $\delta x_t$, the equation above can be written as (after noting that $\dot{\bar{x}}_t = \bar{f}_t - \frac{g^2}{r}G_t$ due to the nominal trajectory $\bar{x}_t$ satisfying the characteristic equation):
\begin{align} \label{x_perturb}
    \dot{\delta x}_t = (\bar{f}_t^x - \frac{g^2}{r} P_t)\delta x_t + O(\delta x_t^2).
\end{align}
Next, we have:
\begin{align}
    \frac{dq}{dt} &= \frac{d}{dt} (G_t+ P_t\delta x_t+\cdots)
    = -l_x - f_x q \nonumber\\
    &= -(\bar{l}_t^x + \bar{l}_t^{xx}\delta x_t+ \cdots) 
    - (\bar{f}_t^x + \bar{f}_t^{xx}\delta x_t+\cdots)(G_t + P_t \delta x_t+ \cdots),
\end{align}
where $\bar{f}_t^{xx} = \frac{\partial^2 f}{\partial x^2}|_{\bar{x}_t}, \bar{l}^x_t = \frac{\partial l}{\partial x}|_{\bar{x}_t},\bar{l}^{xx}_t = \frac{\partial^2 l}{\partial x^2}|_{\bar{x}_t}$.
Using $\frac{d}{dt}P_t \delta x_t = \dot{P}_t \delta x_t + P_t \dot{\delta x}_t$, substituting for $\dot{\delta x}_t$ from \eqref{x_perturb},  and expanding the two sides above in powers of $\delta x_t$ yields:
\begin{align}
    \dot{G}_t + (\dot{P}_t + P_t (\bar{f}_t^x - \frac{g^2}{r} P_t))\delta x_t +\cdots 
    = -(\bar{l}_t^x +\bar{f}_t^x G_t) -(\bar{l}_t^{xx} + \bar{f}_t^x P_t +\bar{f}_t^{xx}G_t)\delta x_t+\cdots.
\end{align}
Equating the first two powers of $\delta x_t$ yields:
\begin{align}
    \dot{G}_t + \bar{l}_t^x + \bar{f}_t^x G_t = 0, \\
    \dot{P}_t + l_t^{xx} + P_t \bar{f}_t^x + \bar{f}_t^x P_t - P_t \frac{g^2}{r} P_t + \bar{f}_{t}^{xx} G_t = 0.
\end{align}
We can see that the first equation for $G_t$ is simply a restatement of the co-state equations in the Minimum Principle. The second equation is a Ricatti-esque equation, except for the second order term $\bar{f}_t^{xx}G_t$. This clearly shows that the feedback design is not an LQR design. The optimal feedback law is given by: $u_t(x_t) = \bar{u}_t + K_t \delta x_t + O(\delta x_t^2)$, where $K_t = -\frac{g}{r}P_t$.\\
Now, we summarize the above development for the general vector case, with a state dependent control influence matrix.
Let the control influence matrix be given as:
$\mathcal{G} = \begin{bmatrix} g_1^1(x) \cdots g_1^p(x)\\ \ddots\\ g_n^1(x) \cdots g_n^p(x) \end{bmatrix} = \begin{bmatrix} \Gamma^1 (x) \cdots \Gamma^p (x)] \end{bmatrix}$, i.e., $\Gamma^j$ represents the control influence vector corresponding to the $j^{th}$ input. Let $\bar{\mathcal{G}}_t = \mathcal{G}(\bar{x}_t)$, where $\{\bar{x}_t\}$ represents the optimal nominal trajectory. Further, let $\mathcal{F} = \begin{bmatrix} f_1(x)\\ \vdots\\ f_n(x)\end{bmatrix}$ denote the drift/ dynamics of the system. Let $G_t = [G_t^1\cdots G_t^n]^{\intercal}$, and $ R^{-1} \bar{\mathcal{G}}_t^{\intercal} G_t = [\bar{u}_t^1 \cdots \bar{u}_t^p]^{\intercal}$, denote the optimal nominal co-state and control vectors respectively. Let $\bar{\mathcal{F}}_t^x = \begin{bmatrix} \frac{\partial f_1}{\partial x_1} \cdots \frac{\partial f_1}{\partial x_n}\\ \ddots\\ \frac{\partial f_n}{\partial x_1} \cdots \frac{\partial f_n}{\partial x_n} \end{bmatrix}|_{\bar{x}_t}$, and similarly $\bar{\Gamma}^{j,x}_t = \nabla_x \Gamma^j|_{\bar{x}_t}$. Further, define: $\bar{\mathcal{F}}_t^{xx,i} = \begin{bmatrix} \frac{\partial^2 f_1}{\partial x_1 \partial x_i} \cdots \frac{\partial^2 f_1}{\partial x_n\partial x_i}\\ \ddots\\ \frac{\partial^2 f_n}{\partial x_1 \partial x_i} \cdots \frac{\partial^2 f_n}{\partial x_n \partial x_i} \end{bmatrix}|_{\bar{x}_t},$ and $\bar{\Gamma}^{j,xx,i}_t$ similarly for the vector function $\Gamma^j$, and $\bar{\mathcal{G}}_t^{x,i} = \begin{bmatrix} \frac{\partial g_1^1}{\partial x_i} \cdots \frac{\partial g_1^p}{\partial x_i}\\ \ddots\\ \frac{\partial g_n^1}{\partial x_i} \cdots \frac{\partial g_n^p}{\partial x_i}\end{bmatrix}|_{\bar{x}_t}$. Finally, define $\mathcal{A}_t = \bar{\mathcal{F}}_t^x + \sum_{j=1}^p \bar{\Gamma}_t^{j,x} \bar{u}_t^j$, $\bar{L}_t^x = \nabla_x l|_{\bar{x}_t}$, and $\bar{L}_t^{xx} = \nabla^2_{xx} l |_{\bar{x}_t}$.
\begin{proposition} \label{T-PFC}
Given the above definitions, the following result holds for the evolution of the co-state/ gradient vector $G_t$, and the Hessian matrix $P_t$, of the optimal cost function ${J}_t(x_t)$, evaluated on the optimal nominal trajectory $\bar{x}_t,t\in[0,T]$:
\begin{align}\label{T-PFC-G}
    \dot{G}_t + \bar{L}_t^x + \mathcal{A}_t G_t = 0,
\end{align}
\begin{multline}\label{T-PFC-P}
    \dot{P}_t + \bar{L}_t^{xx}+ (\mathcal{A}_t + \sum_{j=1}^p \bar{\Gamma}_t^{j,x} \bar{u}_t^j)P_t + P_t(\mathcal{A}_t + \sum_{j=1}^p \bar{\Gamma}_t^{j,x} \bar{u}_t^j)^{\intercal}- P_t\bar{\mathcal{G}}_tR^{-1} \bar{\mathcal{G}}_t^{\intercal}P_t\nonumber\\
    + \sum_{i=1}^n  [\bar{\mathcal{F}}_t^{xx,i} + \sum_{j=1}^p \bar{\Gamma}_t^{j,xx,i} \bar{u}_t^j + \bar{\mathcal{G}}_t^{x,i} \sum_{j=1}^n R^{-1} \bar{\mathcal{G}}_t^{x,j,\intercal} G_t^j]G_t^i = 0,
\end{multline}
with terminal conditions $G_T = \nabla_x c_T|_{\bar{x}_T}$, and $P_t = \nabla_{xx}^2 c_T|_{\bar{x}_T}$
\end{proposition}
\begin{remark} \label{T-PFC-remarks}
\emph{Not LQR.}
The co-state equation \eqref{T-PFC-G} above is identical to the co-state equation in the Minimum Principle \cite{bryson, Pontryagin}. However, the Hessian $P_t$ equation is Ricatti-like with some important differences: note the extra $\sum_j \bar{\Gamma}_t^{j,x} \bar{u}_t^j$ term in the first line, and the second order terms on the last line of the equation stemming from the nonlinear drift and input influence vectors. These terms are not present in the LQR Ricatti equation, and thus, it is clear that this cannot be an LQR, or perturbation feedback design (Ch. 6, \cite{bryson}). Also, if the input influence matrix is independent of the state, then the extra terms in the first line drop out but the second order terms on the last line still remain (as we showed in the scalar case), and hence, it is still different from the LQR case. For the discrete time case with small enough discretization time $\Delta t$, one would simply use the continuous feedback law above with a zero order hold.
\end{remark}
\begin{remark}\label{nonconvex}
\emph{Convexity.} Recall the Lagrange-Charpit equations for solving the HJB \eqref{L-C-1}, \eqref{L-C-2}. Given an unconstrained control, these ODEs have a unique solution for any terminal condition $x_T$ (under standard Lipschitz continuity of the involved functions), and thus, there cannot be two solutions from the nominal terminal state $\bar{x}_T$. Therefore, the open loop optimal trajectory is also the global minimum even though the open loop problem is not convex.
\end{remark}

\subsection{Summary of the Decoupling Results and Implications}
The previous two subsections showed that the deterministic feedback law is an excellent surrogate for the true stochastic feedback law. Further, the feedback parameterization can be written as: $\pi_t(x_t) = \bar{u}_t + K_t \delta x_t$, where $\delta x_t = x_t -\bar{x}_t$ denotes the state deviation from the nominal. Further, it was shown that the optimal open loop sequence $\bar{u}_t$ is independent of the feedback gain, while the feedback gain $K_t$ can be designed based on the optimal $\bar{u}_t$. \textit{Hence, the term decoupling, in the sense that the search for the optimal parameter $(\bar{u}_t^*, K_t^*)$ need not be done jointly, thereby leading to computational tractability.}\\
Moreover, it was shown that depending on how one designed the gain $K_t$, we can obtain $O(\epsilon^4)$ (Proposition \ref{T-PFC}), near-optimality to the true optimal stochastic policy.\\

\subsection{Proof of Lemma 3}
\begin{proof}
We only consider the case when the state $x_t$ is scalar, the vector case is straightforward to derive and only requires a more complex notation.\\
We proceed by induction. The first general instance of the recursion occurs at $t=3$.
It can be shown that: 
\begin{align}
 \delta x_3 = \underbrace{(\bar{A}_2\bar{A}_1(\epsilon w_0) + \bar{A}_2 (\epsilon w_1) + \epsilon w_2)}_{\delta x_3^l} + 
 \underbrace{\{\bar{A}_2 \bar{S}_1(\epsilon w_0) + \bar{S}_2(\bar{A}_1(\epsilon w_0) + \epsilon w_1 + \bar{S}_1(\epsilon w_0))\}}_{e_3}. 
\end{align} 
 Noting that $\bar{S}_1(\cdot)$ and $\bar{S}_2(\cdot)$ are second and higher order terms, it follows that $e_3$ is $O(\epsilon^2)$. \\
 Suppose now that $\delta x_t = \delta x_t^l + e_t$ where $e_t$ is $O(\epsilon^2)$. Then:
\begin{align}
 \delta x_{t+1} = \bar{A}_{t+1}(\delta x_t^l + e_t) + \epsilon w_t + \bar{S}_{t+1}(\delta x_t), 
 = \underbrace{(\bar{A}_{t+1} \delta x_t^l + \epsilon w_t)}_{\delta x_{t+1}^l} +\underbrace{\{\bar{A}_{t+1}e_t + \bar{S}_{t+1}(\delta x_t)\}}_{e_{t+1}}.
 \end{align} 
 Noting that $\bar{S}_{t}$ is $O(\epsilon^2)$ and that $e_{t}$ is $O(\epsilon^2)$ by assumption, the result follows that $e_{t+1}$ is $O(\epsilon^2)$. \\
 Now, let us take a closer look at the term $e_t$ and again proceed by induction. It is clear that $e_1 = e_1^{(2)} =0$. Next, it can be seen that $e_2 = \bar{A}_1e_1^{(2)} + S_1^{(2)}(\delta x_1^l)^2 + O(\epsilon^3) = \bar{S}_1^{(2)} (\epsilon \omega_0)^2 + O(\epsilon^3)$, which shows the recursion is valid for $t=2$ given it is so for $t=1$. \\
 Suppose that it is true for $t$. Then:
\begin{align}
 \delta x_{t+1} = \bar{A}_t \delta x_t + S_t(\delta x_t) + \epsilon \omega_t
& = \bar{A}_t(\delta x_t^l + e_t) + S_t(\delta x_t^l + e_t) + \epsilon \omega _t \\
 & = \underbrace{(\bar{A}_t \delta x_t^l + \epsilon \omega_t)}_{\delta x_{t+1}^l}+ \underbrace{\bar{A}_t e_t^{(2)} + S_t^{(2)}(\delta x_t^l)^2}_{e_{t+1}^{(2)}} + O(\epsilon^3),
\end{align}
 where the last line follows because $e_t = e_t^{(2)} + O(\epsilon^3)$, and $\bar{S}_t(\cdot)$ contains second and higher order terms only. This completes the induction and the proof.
\end{proof}

\subsection{Proof of Lemma 4}
\begin{proof}
We have that:
\begin{align}
J^{\pi} = \sum_t \bar{c}_t + \sum_t \bar{C}_t (\delta x_t^l + e_t) + \sum_t \bar{H}_t(\delta x_t^l + e_t)
= \sum_t \bar{c}_t + \sum_t \bar{C}_t \delta x_t^l + \sum_t \delta x_t^{l'}\bar{H}_t^{(2)} \delta x_t^l + \bar{C}_t e_t^{(2)} + O(\epsilon^3),
\end{align}
where the last line of the equation above follows from an application of Lemma \ref{L1}.
\end{proof}

\subsection{Proof of Proposition 5}
\begin{proof}
We shall show the result for the scalar case for simplicity, the vector state case is relatively straightforward to derive.
We know that any cost function, and hence, the optimal cost-to-go function can be expanded in terms of $\epsilon$ as:
\begin{equation} \label{f1}
J_t(x) = J_t^0 + \epsilon^2 J_t^1 + \epsilon^4 J_t^2 + \cdots% \nonumber
\end{equation}
Thus, substituting the minimizing control in Eq. \ref{opt_control} into the dynamic programming Eq. \ref{DP} implies:
\begin{align}
J_t(x) = \bar{l}(x)\Delta t + \frac{1}{2} r(\frac{-\bar{g}}{r})^2 (J_{t+1}^x)^2 \Delta t + J_{t+1}^x \bar{f}(x)\Delta t  
+ \bar{g}(\frac{-\bar{g}}{r})(J_{t+1}^x)^2 \Delta t+ \frac{\epsilon^2}{2} J_{t+1}^{xx} \Delta t + J_{t+1}(x), \label{f2}
\end{align}
where $J_t^{x}$, and $J_t^{xx}$ denote the first and second derivatives of the cost-to go function. Substituting Eq. \ref{f1} into eq. \ref{f2} we obtain that:
\begin{align}
(J_t^0 + \epsilon^2 J_t^1 + \epsilon^4 J_t^2+\cdots) = \bar{l}(x)\Delta t + 
\frac{1}{2}\frac{\bar{g}^2}{r}(J_{t+1}^{0,x} + \epsilon^2 J_{t+1}^{1,x}+\cdots)^2 \Delta t  
+(J_{t+1}^{0,x}+ \epsilon^2 J_{t+1}^{1,x}+\cdots) \bar{f}(x) \Delta t \nonumber \\
- \frac{\bar{g}^2}{r} (J_{t+1}^{0,x}+ \epsilon^2 J_{t+1}^{1,x}+\cdots)^2\Delta t 
+ \frac{\epsilon^2}{2} (J_{t+1}^{0,x}+ \epsilon^2 J_{t+1}^{1,x}+\cdots)\Delta t + J_{t+1}(x). \label{f3}
\end{align}
Now, we equate the $\epsilon^0$, $\epsilon^2$ terms on both sides to obtain perturbation equations for the cost functions $J_t^0, J_t^1, J_t^2 \cdots$. \\
First, let us consider the $\epsilon^0$ term. Utilizing Eq. \ref{f3} above, we obtain:
\begin{align} \label{f4}
J_t^0  = \bar{l} \Delta t + \frac{1}{2} \frac{\bar{g}^2}{r}(J_{t+1}^{0,x})^2 \Delta t + %\nonumber\\
\underbrace{(\bar{f} + \bar{g}\frac{-\bar{g}}{r} J_t^{0,x})}_{\bar{f}^0} J_t^{0,x}\Delta t + J_{t+1}^0, 
\end{align}
with the terminal condition $J_T^0 = c_T$, and where we have dropped the explicit reference to the argument of the functions $x$ for convenience. \\
Similarly, one obtains by equating the $O(\epsilon^2)$ terms in Eq. \ref{f3} that:
\begin{align}
J_t^1  = \frac{1}{2} \frac{\bar{g}^2}{r} (2J_{t+1}^{0,x}J_{t+1}^{1,x})\Delta t + J_{t+1}^{1,x} \bar{f}\Delta t -\frac{\bar{g}^2}{r} (2J_{t+1}^{0,x}J_{t+1}^{1,x})\Delta t + \frac{1}{2} J_{t+1}^{0,xx} \Delta t + J_{t+1}^1,
\end{align}
which after regrouping the terms yields:
\begin{align} \label{f5}
J_t^1 = \underbrace{(\bar{f}+ \bar{g} \frac{-\bar{g}}{r} J_{t+1}^{0,x})J_{t+1}^{1,x} }_{= \bar{f}^0}\Delta t + \frac{1}{2} J_{t+1}^{0,xx} \Delta t + J_{t+1}^1,
\end{align}
with terminal boundary condition $J_T^1 = 0$.
Note the perturbation structure of Eqs. \ref{f4} and \ref{f5}, $J_t^0$ can be solved without knowledge of $J_t^1, J_t^2$ etc, while $J_t^1$ requires knowledge only of $J_t^0$, and so on. In other words, the equations can be solved sequentially rather than simultaneously.\\

Now, let us consider the deterministic policy $u_t^d(\cdot)$ that is a result of solving the deterministic DP equation:
\begin{equation}
\phi_t(x) = \min_{u} [c(x,u) + \phi_{t+1}(x')],
\end{equation}
where $x' = x + \bar{f}\Delta t + \bar{g} u \Delta t$, i.e., the deterministic system obtained by setting $\epsilon =0$ in Eq. \ref{SDE0}, and $\phi_t$ represents the optimal cost-to-go of the deterministic system. Analogous to the stochastic case, $u_t^d = \frac{-\bar{g}}{r} \phi_t^x$.
Next, let $\varphi_t$ denote the cost-to-go of the deterministic policy $u_t^d(\cdot)$ \textit{when applied to the stochastic system, i.e., Eq. \ref{SDE0} with $\epsilon >0$}. Then, the cost-to-go of the deterministic policy, when applied to the stochastic system, satisfies:
\begin{equation}
\varphi_t = c(x, u_t^d(x)) + E[\varphi_{t+1}(x')],
\end{equation}
where $x' = \bar{f}\Delta t + \bar{g}u_t^d \Delta t + \epsilon\sqrt{\Delta t}\omega_t$. Substituting $u_t^d(\cdot) = \frac{-\bar{g}}{r}\phi_t^x$ into the equation above implies that:
\begin{align}
\varphi_t &= \varphi_t^0 + \epsilon^2\varphi_t^1 + \epsilon^4 \varphi_t^2+ \cdots \nonumber\\
&= \bar{l} \Delta t + \frac{1}{2}\frac{\bar{g}^2}{r}(\phi_{t+1}^x)^2 \Delta t \nonumber
+ (\varphi_{t+1}^{0,x} + \epsilon^2\varphi_{t+1}^{1,x} + \cdots )\bar{f} \Delta t 
+  \bar{g}\frac{-\bar{g}}{r} \phi_{t+1}^x (\varphi_{t+1}^{0,x} + \epsilon^2\varphi_{t+1}^{1,x} + \cdots ) \Delta t \nonumber\\
&~~~~~~~~~~~~~~~~~~~~+ \frac{\epsilon^2}{2} (\varphi_{t+1}^{0,xx} + \epsilon^2\varphi_{t+1}^{1,xx} + \cdots ) \Delta t 
+  (\varphi_{t+1}^0 + \epsilon^2\varphi_{t+1}^1 + \cdots). \label{f6}
\end{align}
As before, if we gather the terms for $\epsilon^0$, $\epsilon^2$ etc. on both sides of the above equation, we shall get the equations governing $\varphi_t^0, \varphi_t^1$ etc.  First, looking at the $\epsilon^0$ term in Eq. \ref{f6}, we obtain:
\begin{align} \label{f7}
\varphi_t^0 = \bar{l} \Delta t + \frac{1}{2} \frac{\bar{g}^2}{r}(\phi_{t+1}^x)^2 \Delta t  %\nonumber\\
+ (\bar{f} + \bar{g} \frac{-\bar{g}}{r}\phi_{t+1}^x )\varphi_{t+1}^{0,x}\Delta t  + \varphi_{t+1}^0,    
\end{align}
with the terminal boundary condition $\varphi_T^0 = c_T$. However, the deterministic cost-to-go function also satisfies:
\begin{align}\label{f8}
\phi_t = \bar{l} \Delta t + \frac{1}{2} \frac{\bar{g}^2}{r} (\phi_{t+1}^x)^2 \Delta t  %\nonumber\\
+( \bar{f}   + \bar{g} \frac{-\bar{g}}{r} \phi_{t+1}^x) \phi_{t+1}^x \Delta t  + \phi_{t+1},
\end{align}
with terminal boundary condition $\phi_T = c_T$. Comparing Eqs. \ref{f7} and \ref{f8}, it follows that $\phi_t = \varphi_t^0$ for all $t$. Further, comparing them to Eq. \ref{f4}, it follows that $\varphi_t^0 = J_t^0$, for all $t$. Also, note that the closed loop system above, $\bar{f}   + \bar{g} \frac{-\bar{g}}{r} \phi_{t+1}^x = \bar{f}^0$ (see Eq. \ref{f4} and \ref{f5}). \\

Next let us consider the $\epsilon^2$ terms in Eq. \ref{f6}. We obtain:
\begin{align}
\varphi_t^1 = \bar{f} \varphi_{t+1}^{1,x} \Delta t + \bar{g}\frac{-\bar{g}}{r} \phi_{t+1}^x \varphi_{t+1}^{1,x} \Delta t + \nonumber
\frac{1}{2}\varphi_{t+1}^{0,xx} + \varphi_{t+1}^1.
\end{align}
Noting that $\phi_t = \varphi_t^0 $, implies that (after collecting terms):
\begin{align} \label{f9}
\varphi_t^1 = \bar{f}^0 \varphi_{t+1}^{1,x} \Delta t + \frac{1}{2}\varphi_{t+1}^{0,xx} \Delta t + \varphi_{t+1}^1,
\end{align}
with terminal boundary condition $\varphi_N^1 = 0$. Again, comparing Eq. \ref{f9} to Eq. \ref{f5}, and noting that $\varphi_t^0 = J_t^0$,  it follows that $\varphi_t^1 = J_t^1$, for all $t$. This completes the proof of the result. 
\end{proof}


==> Algorithm.tex <==
\section{Decoupled Data Based Control (D2C) Algorithm}\label{sec4}

In this section, we proposed a novel decoupled data based control (D2C) algorithm formalizing  the ideas proposed in Section \ref{sec3}. First, a noiseless open-loop optimization problem is solved to find a nominal optimal trajectory. Then a linearized closed-loop controller is designed around this nominal trajectory, such that, with existence of stochastic perturbations, the state stays close to the optimal open-loop trajectory. The three-step framework to solve the stochastic feedback control problem may be summarized as follows.
\begin{itemize}
\item Solve the open loop optimization problem using gradient descent with a black box simulation model of the dynamics.
\item Linearize the system around the open loop optimal trajectory and identify the linearized time-varying system from experimental data. 
\item Design an LQR controller which results in an optimal linear control policy around the nominal trajectory. 
\end{itemize}
In the following section, we discuss each of the above steps.

\subsection{Open Loop Trajectory Optimization}
\label{sec_open}
A first order gradient descent method is used here for the open loop optimization problem given in \eqref{OL}, where the underlying dynamic model is used as a blackbox, and the necessary gradients are found from a sequence of input perturbation experiment data using standard least square.

Denote  the initial guess of the control sequence as $U^{(0)} = \{\bar{u}_t^{(0)} \}_{t = 1}^{T}$, and  the corresponding  states $\mathcal{X}^{(0)} = \{\bar{x}_t^{(0)} \}_{t=1}^T$. The control policy is updated iteratively via
\begin{align}\label{ctrl_upd}
U^{(n + 1)} = U^{(n)} - \alpha \nabla_U \bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}},
\end{align}
where $U^{(n)} = \{\bar{u}_t^{(n)} \}_{t = 1}^{T}$ denotes the control sequence in the $n^{th}$ iteration, $\mathcal{X}^{(n)} = \{\bar{x}_t^{(n)}\}_{t=1}^{T}$ denotes the corresponding states, and $\alpha$ is the step size parameter. As $\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}$ is the expected cumulative cost under control sequence $U^{(n)}$ and corresponding states $\mathcal{X}^{(n)}$, the gradient vector is defined as
$%$\begin{align}\label{gradv}
\nabla_U \bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}} = \begin{pmatrix} \frac{\partial \bar{J}}{\partial u_1} & \frac{\partial \bar{J}}{\partial u_1} & \cdots & \frac{\partial \bar{J}}{\partial u_{T}} \end{pmatrix}|_{\mathcal{X}^{(n)}, U^{(n)}},
$%\end{align}
which is the gradient of the expected cumulative cost w.r.t the control sequence after $n$ iterations. The following paragraph elaborates on how to estimate the above gradient. 

Let us define a rollout to be an episode in the simulation that starts from the initial settings to the end of the horizon with a control sequence. For each iteration, multiple rollouts are conducted sequentially with both the expected cumulative cost and the gradient vector updated iteratively after each rollout. During one iteration for the control sequence, the expected cumulative cost is calculated as
$%$\begin{align}\label{cost_ite}
\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{j+1} = 
(1-\frac{1}{j})\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{j} +  \frac{1}{j}(J|_{\mathcal{X}^{j,(n)}, U^{j,(n)}}),
$%\end{align}
where $j$ denotes the $j^{th}$ rollout within the current iteration process of control sequence. $\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{j}$ is the expected cumulative cost after $j$ rollouts while $J|_{\mathcal{X}^{j,(n)}, U^{j,(n)}}$ denotes the cost of the $j^{th}$ rollout under control sequence $U^{j,(n)}$ and corresponding states $\mathcal{X}^{j,(n)}$. Note that $U^{j,(n)} = \{\bar{u}_t^{(n)} + \delta u^{j,(n)}_t\}_{t = 1}^{T}$ where $\{\delta u^{j,(n)}_t\}^T_{t=1}$ is the zero-mean, i.i.d Gaussian noise added as perturbation to the control sequence $U^{(n)}$.

Then the gradient vector is calculated in a similar sequential manner as
$%$\begin{align}\label{grad_ite}
\nabla_U\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{j+1} = 
(1-\frac{1}{j})\nabla_U\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{j} + \nonumber\\ \frac{1}{j\sigma_{\delta u}}(J|_{\mathcal{X}^{j,(n)}, U^{j,(n)}}-\bar{J}|_{\mathcal{X}^{(n)},U^{(n)}}^{j+1})(U^{j,(n)}-U^{(n)}),
$%\end{align}
where $\sigma_{\delta u}$ is the variance of the control perturbation and $\nabla_U\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{j+1}$ denotes the gradient vector after $j$ rollouts. Note that after each rollout, both the expected cumulative cost and the gradient vector are updated. The rollout number $m$ in one iteration for the control sequence is decided by the convergence of both the expected cumulative cost and the gradient vector. After $m$ rollouts, the control sequence is updated by equation (\ref{ctrl_upd}) in which $\nabla_U \bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}$ is estimated by $\nabla_U\bar{J}|_{\mathcal{X}^{(n)}, U^{(n)}}^{m}$. Keep doing this until the cost converges and the optimized nominal control sequence is $ \{\bar{u}^*_t\}_{t = 1}^{T}=\{\bar{u}^{(N-1)}_t\}_{t = 1}^{T}$.

Higher order approaches other than gradient descent are possible. However, for a general system, the gradient descent approach is easy to implement. Also it is memory efficient and highly amenable to parallelization as a result of our sequential approach.

\subsection{Linear Time-Varying System Identification}
\label{sec_ls}
Closed loop control design  specified in \eqref{CL} or the approximate closed loop control design specified in \eqref{eq:acl1} requires the knowledge of the parameters $A_{t}, B_{t}, 1 \leq t \leq T,$ of the perturbed linear system. We propose a linear time variant (LTV) system identification procedure to estimate these parameters.  

First start from perturbed linear system given by equation \eqref{eq:acl1}. Using only first order information and estimate the system parameters $A_{t}, B_{t}$ with the following form
$%$\begin{align}
%\label{est_sys}
 \delta x_{t+ 1} = \hat{A_t} \delta x_t+\hat{B_t} \delta u_t,
$%\end{align}
rewrite with augmented matrix
$%$\begin{align}
%\label{aug system}
 \delta x_{t+ 1} = [\hat{A_t} ~|~ \hat{B_t}]  ~
\begin{bmatrix}
   \delta x_t \\
   \delta u_t \\
\end{bmatrix},
$%\end{align}
Now write out their components for each iteration in vector form as,
$%$\begin{align}
%\label{lsq1}
 Y = [\delta x_{t+1}^0 \delta x_{t+1}^1 \cdots \delta x_{t+1}^{N-1}],\nonumber\\
 X=\begin{bmatrix}
   \delta x_t^0 & \delta x_t^1& \cdots & \delta x_t^{N-1} \\
   \delta u_t^0 &  \delta u_t^1 & \cdots & \delta u_t^{N-1} \\
\end{bmatrix},\nonumber\\
  Y=[\hat{A_t} ~|~ \hat{B_t}]X,
$%\end{align}
where N is the total iteration number. $\delta x_{t+1}^n$ denotes the output state deviation , $\delta x_{t}^n$ denotes the input state perturbations and $\delta u_{t}^n$ denotes the input control perturbations at time $t$ of the $n^{th}$ iteration. All the perturbations are zero-mean, i.i.d, Gaussian random vectors whose covariance matrix is $\sigma I$ where  I is the identity matrix and $\sigma $ is a scalar. Note that here one iteration only has one rollout.

The next step is to apply the perturbed control $\{\bar{u}^*_t + \delta u_t^n\}_{t = 1}^{T}$ to the system and collect input-output experiment data in a blackbox simulation manner.

Using the  least square method $\hat{A_t}$ and $\hat{B_t}$ can be calculated in the following procedure
$%$\begin{align}
%\label{lsq2}
 YX'=[\hat{A_t} ~|~ \hat{B_t}]XX'.
$%\end{align}
Here $X'$ is the transpose of $X$.
As the perturbations are zero-mean, i.i.d, Gaussian random noise, $XX' = \sigma NI$. Then
$%$\begin{align}
%\label{lsq3}
 [\hat{A_t} ~|~ \hat{B_t}] = \frac{1}{\sigma N}YX'. %\nonumber \\
$%\end{align}
%  &=\frac{1}{\sigma N}[\delta x_{t+1}^0 \delta x_{t+1}^1 \cdots \delta x_{t+1}^{N-1}]
% \begin{bmatrix}
%   (\delta x_t^0)' &  (\delta u_t^0)'\\
%   (\delta x_t^1)' &  (\delta u_t^1)'\\
%   \vdots & \vdots \\
%   (\delta x_t^{N-1})' &  (\delta u_t^{N-1})'\\
% \end{bmatrix}


The calculation procedure can also be done in a sequential way similar to the update of the gradient vector in the open-loop optimization algorithm. Therefore it is highly amenable to parallelization and memory efficient.

\subsection{Closed Loop Control Design} 
Given the parameter estimate of the perturbed linear system, we solve the  closed loop control problem given in \eqref{eq:acl1}. This is a standard LQR problem. By solving the Riccati equation, we can get the closed-loop optimal feedback gain $K^*_t$. The detail of the design is standard and omitted here. 

\begin{algorithm}
    \caption{D2C Algorithm}
    \label{algo1}
   {\bf 1)}  Solve the deterministic open-loop optimization problem for optimal open loop nominal control sequence and trajectory $(\{\bar{u}^*_t\}_{t = 1}^{T}, \{\bar{x}_t^*\}_{t = 1}^T)$ using gradient descent method (Section \ref{sec_open}).\\
  {\bf 2)} Identify the LTV system $(\hat{A}_t, \hat{B}_t)$ via least square estimation (Section \ref{sec_ls}).\\
  {\bf 3)} Solve the Riccati equations  using estimated LTV system equation for feedback gain $\{ K^*_t \}_{t = 1}^{T}$.\\
  {\bf 4)} Set $t = 1$, given initial state $x_1 = \bar{x}_1^*$ and state deviation $\delta x_1 = 0$.\\
\While{$t \leq T$}{
  \begin{align}
& u_t = \bar{u}_t^* + K^*_t \delta x_t, \nonumber \\
& x_{t + 1} = f(x_{t}) + B_{t} (u_{t} + \epsilon w_{t}),\nonumber \\
& \delta x_{t+1} = x_{t + 1}-\bar{x}^*_{t + 1}
\end{align}
 $t = t + 1$.
}
\end{algorithm}

\subsection{D2C Algorithm: Summary}
The Decoupled Data Based Control  (D2C) Algorithm is summarized in Algorithm \ref{algo1}. 






==> Discussion.tex <==
\section{DISCUSSION}
%In this section, we present a detailed analysis of  drawing from the intersection between traditional stochastic optimal control and RL.

From the above training plots, it is clear that our D2C approach
learns the open-loop optimal policy much faster than DDPG. As the system identification and feedback gain calculation take only a small portion of time, the total time comparison in (TABLE-\ref{timecompare}) shows that D2C greatly improves the data efficiency.

From the above performance comparison plots, the D2C approach has lower error under certain noise level, which shows that D2C improves the robustness of the closed-loop system compared with DDPG. However, it may be noted the error variance of D2C increased abruptly when the noise level is higher than a threshold and drives the system too far away from the nominal trajectory that the LQR controller can't fix it. This could be considered a drawback for D2C. 
%Although continuous RL algorithms such as DDPG learn the policy and thereby interpolated to the entire state space, we consider the task in a limited timeframe window approach. 

Adv.

The training time is often ignored in comparing the RL algorithm
DDPG has no guarantees..involves trial and error tuning, reward shaping
Our method can scale-up to higher dimensional state-space without any knowledge about the system's dynamical model.

Another disadvantage with D2C over canonical RL algorithms is that the cost could be stuck in a local minimum whereas DDPG, due to the nature of stochastic gradient descent in training neural networks, can reach the global optimum. 


==> Simulations.tex <==
\section{Simulation Results}\label{sec5}
In this section, we compare the D2C approach with the well-known deep reinforcement learning algorithm - Deep Deterministic Policy Gradient (DDPG)  \citep{DDPG}. For the comparison, we evaluate both the methods in the following three aspects:  \\
%\begin{itemize}
\textit{Data efficiency in training} - the amount of data sampling and storage required to achieve a desired task.\\
\textit{Robustness to noise}- the deviation from the predefined task due to random noise in process in the testing stage.\\
\textit{Ease of training} - the challenges involved in training with either of the data-based approaches.
%\end{itemize}
    

\subsection{Tasks and Implementation}
We tested our method with four  benchmark tasks, all implemented in MuJoCo simulator \citep{mujoco}: Inverted pendulum, Cart-pole, 3-link swimmer and 6-link swimmer \citep{dpmd_suite}. Each of the systems and their tasks are briefly defined as follows:\\
\textbf{Inverted pendulum} A swing-up task of this 2D system from its downright initial position is considered. \\
\textbf{Cart-pole} 
The state of a 4D under-actuated cart-pole comprises the angle of the pole, cart's horizontal position and their rates. Within a given horizon, the task is to swing-up the pole and balance it at the middle of the rail by applying a horizontal force on the cart.\\
\textbf{3-link Swimmer} 
The 3-link swimmer model has 5 degrees of freedom and together with their rates, the system is described by 10 state variables. The task is to solve the planning and control problem from a given initial state to the goal position located at the center of the ball. Controls can only be applied in the form of torques to two joints. Hence, it is under-actuated by 3 DOF.\\
\textbf{6-link Swimmer} 
The task with a 6-link swimmer model is similar to that defined in the 3-link case. However, with 6 links, it has 8 degrees of freedom and hence, 16 state variables, controlled by 5 joint motors. \\


\begin{figure*}[!htb]
\begin{multicols}{4}
    \hspace{0.5cm}    
    \subfloat[Inverted Pendulum - D2C]{\includegraphics[width=1\linewidth]{Images/Examples/D2C/Inverted_pendulum/d2c_openloop_invertedpendulum.png}}
     \subfloat[Cart-Pole - D2C]{\includegraphics[width=\linewidth]{Images/Examples/D2C/Cart_pole/d2c_openloop_cartpole.png}}
     \subfloat[3-link Swimmer - D2C]{\includegraphics[width=\linewidth]{Images/Examples/D2C/Swimmer_3_link/d2c_openloop_swimmer3.png}}
     \subfloat[6-link Swimmer - D2C]{\includegraphics[width=\linewidth]{Images/Examples/D2C/Swimmer_6_link/d2c_openloop_swimmer6.png}}
     
    \end{multicols}
\begin{multicols}{4} 
    \hspace{0.5cm}    
      \subfloat[Inverted Pendulum - DDPG]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Inverted_pendulum/training_cost_fraction.png}}
      \subfloat[Cart-Pole - DDPG]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Cart_pole/training_reward_fraction.png}}
      \subfloat[3-link Swimmer - DDPG]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Swimmer_3_link/training_episodic_reward_fraction.png}}
      \subfloat[6-link Swimmer - DDPG]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Swimmer_6_link/swimming_6_training_reward.png}}
\end{multicols}
%\vspace{.3in}
\caption{Episodic reward fraction vs time taken during training}
\end{figure*}

\begin{figure*}[!htb]
\begin{multicols}{4}
    \hspace{0.5cm}    
      \subfloat[Inverted Pendulum]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Inverted_pendulum/testing_terminal_mse_D2C_DDPG.png}}    
      \subfloat[Cart-Pole ]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Cart_pole/terminal_mse_D2C_DDPG.png}}
      \subfloat[3-link Swimmer]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Swimmer_3_link/terminal_mse_D2C_DDPG.png}}
      \subfloat[6-link Swimmer ]{\includegraphics[width=\linewidth]{Images/Examples/DDPG/Swimmer_6_link/swimmer_6_terminal_mse_D2C_DDPG.png}}
\end{multicols}
%\vspace{.3in}
\caption{Terminal MSE vs noise level during testing}
\end{figure*} 

D2C implementation is done in three stages corresponding to those mentioned in the previous section and `MuJoCo Pro 150' is used as the environment for simulating the blackbox model. An off-the-shelf implementation of DDPG provided by {\it Keras-RL} \citep{plappert2016kerasrl} library has been customized for our simulations. It may be noted that the structure of the reward function is formulated to optimize the performance of DDPG and hence, different from that used in D2C. However, the episode length (or horizon) and the time-discretization step is held identical. Although continuous RL algorithms such as DDPG learn the policy and thereby interpolating it to the entire state space, we consider the task-based experiments in a finite limited time-frame window approach. Training is performed until the neural networks' loss is converged. Hence, though the episodic reward does seem to converge earlier, that itself may not indicate that the policy is converged. 

For a fair comparison, `Episodic reward/cost fraction' is considered with both methods. It is defined as the fraction of reward obtained in an episode during training w.r.t the nominal episodic reward (converged reward). Note that the words 'reward' and 'cost' are being used interchangeably due to their different notions in optimal control and RL literature respectively, though they achieve the same objective. For simplicity, one is considered the negative of the other. 



\subsection{Performance Comparison}

{\bf Data-efficiency:} As mentioned above, efficient training is one that requires minimal data sampling in order to achieve the same behavior. One way of measuring it is to collate the times taken for the episodic cost (or reward) to converge during training. Plots in Fig. 1 show the training process with both methods on the systems considered. Table \ref{timecompare} delineates the times taken for training respectively. As the system identification and feedback gain calculation in case of D2C take only a small portion of time, the total time comparison in (Table \ref{timecompare}) shows that D2C learns the optimal policy substantially faster  than DDPG and hence, has a better data efficiency. 

{\bf Robustness to noise:} As with canonical off-policy RL algorithms, DDPG requires that an exploration noise be added to the policy, during training. Given that the training adapts the policy to various levels of noise, combined with hours of intense training and a nonlinear policy output, it is expected that it is more robust towards noise as is evident from Figs. 2 (c) and 2 (d). However, from plots in Figs. 2 (a) and (b), it is evident that in some systems the performance of D2C is on par with or better than DDPG. 
It may also be noted that the error variance in D2C method increases abruptly when the noise level is higher than a threshold and drives the system too far away from the nominal trajectory that the LQR controller cannot fix it. This could be considered a drawback for D2C. However, it must be noted that the range of noise levels (up until 100 \% of the maximum control signal) that we are considering here is far beyond what is typically encountered in practical scenarios. Hence, even in swimmer examples, the performance of D2C is tolerable to a reasonable extent of noise in the system.

{\bf Ease of training:} The ease of training is often an ignored topic in analyzing a reinforcement learning (RL) algorithm. By this, we mean the challenges associated with its implementation. As with many RL algorithms that involve neural networks, DDPG has no guarantees for policy convergence. As a result, the implementation often involves tuning a number of hyper-parameters and a careful reward shaping in a trial and error fashion, which is even more time-consuming given that their successful implementation already involves significant time and computational resources. Reproducibility \citep{henderson2018deep} is still a major challenge that RL is yet to overcome. On the other hand, training in our approach is predictable and very reliable.

To elucidate the ease of training from an empirical perspective, the exploration noise that is required for training in DDPG mandates the system to operate with a shorter time-step than a threshold, beyond which the simulation fails due to an unbearable magnitude of control actions into the system. For this, we train both the swimmers in one such case (with $\Delta t = 0.01$ sec) till it fails and execute the intermediate policy. Fig. \ref{testing_mse_001_swimmers} shows the plot in the testing-stage with both methods. It is evident from the terminal state mean-squared error at zero noise level that the nominal trajectory of DDPG is incomplete and its policy failed to reach the goal. The effect is more pronounced in the higher-dimensional 6-link swimmer system (Fig. \ref{testing_mse_001_swimmer6}), where the DDPG's policy can be deemed to be downright broken. Note, from Table \ref{timecompare}, that the systems have been trained with DDPG for a time that is more than thrice with the 3-link swimmer and 4 times with the 6-link swimmer. On the other hand, under the same conditions, the seamless training of D2C results in a working policy with even greater data-efficiency.    


%The fundamental differences in both the algorithms arise from their distinct formulations, as in, finite-horizon in case of D2C and an infinite-horizon problem in DDPG. From optimal control literature, it is well-known that the terminal cost in a finite-horizon problem plays a crucial role in stabilizing the system \citep{}. Hence, methods such as D2C are able to achieve their goals accurately whereas DDPG consumes an inordinate amount of time in 'fine-tuning' their behavior towards the goal. However, we also note DDPG explores the entire state-space and can result in a generic policy. Another drawback with D2C over canonical RL algorithms is that the cost could be stuck in a local minimum, whereas DDPG due to the nature of stochastic gradient descent in training neural networks, can potentially reach the global optimal solution. Nevertheless, we hope that our approach signifies the potential of decoupling based approaches such as D2C in a reinforcement learning paradigm and recognizes the need for more hybrid approaches that complement the merits of each.


\begin{table}[h]
\caption{Simulation Parameters and Training Outcomes} \label{timecompare}
\begin{center}
\setlength{\tabcolsep}{0.6mm}{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{System}&\textbf{Steps}& \textbf{Time-}& \multicolumn{3}{|c|}{\textbf{Training time (sec.)}}\\\cline{4-6}
&\textbf{per}&\textbf{step}&\multicolumn{2}{|c|}{\textbf{D2C}}& \\\cline{4-5}
&\textbf{episode}&\textbf{(sec.)}& \textbf{Open-}& \textbf{Closed-}&\textbf{DDPG}\\
&&&\textbf{loop}&\textbf{loop}&\\
\hline
Inverted& 30 & 0.1 &12.9  &$<0.1$& 2261.15\\
Pendulum& & & & &\\
\hline
Cart pole& 30 & 0.1 & 15.0 & 1.33& 6306.7\\
\hline
3-link & 1600& 0.005 & 7861.0&13.1 & 38833.64\\
Swimmer&  800& 0.01 & 4001.0&4.6 & 13280.7*\\
\hline
6-link &1500 & 0.006 &9489.3&26.5 & 88160\\
Swimmer &900 & 0.01 &3585.4&16.4 & 15797.2*\\ 
\hline
\end{tabular}
}
\end{center}
\end{table}


\begin{figure}
     \centering
     \subfloat[3-link swimmer]
     {\includegraphics[width=0.23\textwidth]{Images/Examples/DDPG/Swimmer_3_link/testing_mse_swimmer_001_noise_d2c_ddpg.png}
     \label{testing_mse_001_swimmer}}
     \subfloat[6-link swimmer]
     {\includegraphics[width=0.23\textwidth]{Images/Examples/DDPG/Swimmer_6_link/testing_mse_001_d2c_ddpg_swimmer6.png}
     \label{testing_mse_001_swimmer6}}
     \caption{D2C vs DDPG at $\Delta t = 0.01 s$}
     %\vspace{.3in}
     \label{testing_mse_001_swimmers}
\end{figure}

